Contextual bandits with entropy-based human feedback

In recent years, preference-based human feedback mechanisms have become essential for enhancing model performance across diverse applications, including conversational AI systems such as ChatGPT. However, existing approaches often neglect critical aspects, such as model uncertainty and the variability in feedback quality. To address these challenges, we introduce an entropy-based human feedback framework for contextual bandits, which dynamically balances exploration and exploitation by soliciting expert feedback only when model entropy exceeds a predefined threshold. Our method is model-agnostic and can be seamlessly integrated with any contextual bandit agent employing stochastic policies. Through comprehensive experiments, we show that our approach achieves significant performance improvements while requiring minimal human feedback, even under conditions of suboptimal feedback quality. This work not only presents a novel strategy for feedback solicitation but also highlights the robustness and efficacy of incorporating human guidance into machine learning systems. Our code is publicly available: https://github.com/BorealisAI/CBHF

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> sections/checklist.tex <==
\newpage
\section*{NeurIPS Paper Checklist}

%%% BEGIN INSTRUCTIONS %%%
The checklist is designed to encourage best practices for responsible machine learning research, addressing issues of reproducibility, transparency, research ethics, and societal impact. Do not remove the checklist: {\bf The papers not including the checklist will be desk rejected.} The checklist should follow the references and precede the (optional) supplemental material.  The checklist does NOT count towards the page
limit. 

Please read the checklist guidelines carefully for information on how to answer these questions. For each question in the checklist:
\begin{itemize}
    \item You should answer \answerYes{}, \answerNo{}, or \answerNA{}.
    \item \answerNA{} means either that the question is Not Applicable for that particular paper or the relevant information is Not Available.
    \item Please provide a short (1–2 sentence) justification right after your answer (even for NA). 
   % \item {\bf The papers not including the checklist will be desk rejected.}
\end{itemize}

{\bf The checklist answers are an integral part of your paper submission.} They are visible to the reviewers, area chairs, senior area chairs, and ethics reviewers. You will be asked to also include it (after eventual revisions) with the final version of your paper, and its final version will be published with the paper.

The reviewers of your paper will be asked to use the checklist as one of the factors in their evaluation. While "\answerYes{}" is generally preferable to "\answerNo{}", it is perfectly acceptable to answer "\answerNo{}" provided a proper justification is given (e.g., "error bars are not reported because it would be too computationally expensive" or "we were unable to find the license for the dataset we used"). In general, answering "\answerNo{}" or "\answerNA{}" is not grounds for rejection. While the questions are phrased in a binary way, we acknowledge that the true answer is often more nuanced, so please just use your best judgment and write a justification to elaborate. All supporting evidence can appear either in the main paper or the supplemental material, provided in appendix. If you answer \answerYes{} to a question, in the justification please point to the section(s) where related material for the question can be found.
\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We showcase that we (1) are able to incorporate HF into a CB setting and that our proposed entropy-based criterion functions as intended in the experiments section.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We discuss the limitations at the end of the paper.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate "Limitations" section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory Assumptions and Proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: There are no theoretical results. We propose a criteria that is well justified based on related literature.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental Result Reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We discuss datasets, experiments and hyperparameters. We also release code.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Code released, data is open source.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental Setting/Details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The hyperparameters are specified. The splits and other parts are standard and based on cited papers.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment Statistical Significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerNo{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We do not report error bars, but the results are sufficiently distinct that there is no ambiguity on the best performing method.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
        \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments Compute Resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We use single GPUs, and our experiments could be reproduced using minimal resources.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code Of Ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: There are no breaches of ethics. We are conducting analyses of bandit settings with human feedback. All of our experiments are within the guidelines.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader Impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: There is no potential for negative societal impacts beyond those linked to using bandit systems in general.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that there is no societal impact of the work performed.
        \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We use abstract theoretical and well-benchmarked datasets. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The associated code has all the necessary licenses on a file-per-file and dataset basis.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New Assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: There are no assets.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and Research with Human Subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: No crowd-sourcing or human subjects. The "human feedback" collected is based on ML systems. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional Review Board (IRB) Approvals or Equivalent for Research with Human Subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: See above.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\end{enumerate}

==> sections/cost_modeling.tex <==

\section{Detailed Analysis of Feedback Solicitation Costs and Their Impact on Cumulative Rewards}

In systems that integrate human feedback, the cost of feedback solicitation plays a crucial role in determining the efficiency and practicality of the algorithm. Below, we provide a structured analysis of these costs and their effects.

\subsection{Cost Components in Feedback Solicitation}

Feedback solicitation costs can be broken into three primary components:
\begin{itemize}
    \item \textbf{Human Effort Cost (\(C_h\))}: Time, cognitive load, or financial compensation required for a human expert to provide feedback.
    \item \textbf{System Overhead (\(C_s\))}: Computational and communication overhead associated with querying, collecting, and processing feedback.
    \item \textbf{Opportunity Cost (\(C_o\))}: Delay or missed opportunities to explore other actions during feedback solicitation.
\end{itemize}

The total cost per solicitation can be expressed as:
\[
C_{\text{total}} = C_h + C_s + C_o.
\]

\subsection{Trade-off Between Feedback and Performance}

Feedback improves learning by reducing uncertainty in decision-making but comes at a cost. The trade-off is evident in two opposing factors:
\begin{itemize}
    \item \textbf{Benefits}: Incorporating feedback accelerates convergence, reduces regret, and improves cumulative rewards.
    \item \textbf{Costs}: Frequent feedback queries increase the total cost, potentially diminishing the system’s overall utility.
\end{itemize}

The cumulative rewards \(R_T\) after \(T\) rounds with feedback solicitation frequency \(p\) can be modeled as:
\[
R_T = \sum_{t=1}^T r_t - p \cdot C_{\text{total}},
\]
where \(r_t\) represents the reward at time step \(t\), and \(p\) is the fraction of rounds in which feedback is solicited.

\subsection{Effect of Feedback Quality and Frequency}

\subsubsection{High-Quality Feedback (\(q_t \to 1\))}

\begin{itemize}
    \item \textbf{Impact}: High-quality feedback significantly reduces regret, as the system quickly learns optimal actions.
    \item \textbf{Cost Justification}: Even with higher solicitation costs, the performance gains justify frequent feedback, especially in complex environments.
\end{itemize}

\subsubsection{Low-Quality Feedback (\(q_t \to 0\))}

\begin{itemize}
    \item \textbf{Impact}: Low-quality feedback adds noise to the learning process, diminishing performance gains.
    \item \textbf{Cost Justification}: Frequent solicitation becomes inefficient, and selective feedback solicitation based on entropy thresholds (\(\lambda\)) is preferred.
\end{itemize}

\subsubsection{Frequency of Feedback (\(p\))}

\begin{itemize}
    \item High \(p\) improves learning but incurs higher total costs, leading to diminishing returns as cumulative rewards plateau.
    \item Low \(p\) reduces costs but risks slower convergence and higher regret.
\end{itemize}

\subsection{Entropy-Based Feedback Solicitation}

An entropy-based mechanism optimizes feedback solicitation by querying only when the model’s uncertainty surpasses a predefined threshold (\(\lambda\)):
\begin{itemize}
    \item \textbf{High Entropy (\(H(\pi) > \lambda\))}: Feedback is requested to resolve uncertainty, ensuring maximum utility from the cost incurred.
    \item \textbf{Low Entropy (\(H(\pi) \leq \lambda\))}: Feedback is avoided as the model is confident in its decision.
\end{itemize}

This selective querying strategy reduces the total feedback cost while maintaining performance by focusing resources where they have the highest impact.

\subsection{Experimental Analysis}

Using simulated environments:
\begin{itemize}
    \item \textbf{Performance vs. Cost}: Reducing feedback frequency (\(p\)) by increasing \(\lambda\) leads to a marginal decrease in performance while significantly reducing costs. For instance, at \(p = 0.3\), performance dropped by only 5\% compared to \(p = 1.0\), but the cost was reduced by 70\%.
    \item \textbf{Dataset Dependency}: Feedback efficiency varies across datasets. Datasets with large action spaces benefit more from frequent feedback (e.g., Delicious dataset), while datasets with fewer actions (e.g., Bibtex dataset) require less frequent feedback due to faster convergence.
\end{itemize}

\subsection{Insights and Practical Implications}

\begin{itemize}
    \item \textbf{Optimal Feedback Strategy}: Use selective feedback based on model uncertainty and adjust \(\lambda\) to balance feedback costs with performance gains depending on the application.
    \item \textbf{Recommendations for Practitioners}: In high-cost settings, prioritize low feedback frequency (\(p \to 0.2-0.4\)) with robust entropy thresholds. For critical applications, higher feedback costs can be justified for improved cumulative rewards.
    \item \textbf{Scalability}: Entropy-based solicitation is particularly effective for large-scale systems where querying all rounds is impractical.
\end{itemize}

\subsection{Conclusion}

Balancing feedback solicitation costs and cumulative rewards requires careful tuning of feedback frequency and quality thresholds. An entropy-based approach effectively minimizes costs while maintaining performance, making it a practical solution for real-world applications. Future work could explore dynamic threshold adaptation to further optimize this trade-off.



==> sections/experiments_improved_method.tex <==
\section{Experiments for Hybrid Feedback Mechanism}

\subsection{Synthetic Dataset Construction}

To evaluate the proposed \textbf{HybridLinearBandit} method, we constructed a synthetic dataset simulating a recommendation environment. The dataset includes:

- \textbf{Contextual Features}:
  - Each context \(\mathbf{x}_t \in \mathbb{R}^d\) represents the feature vector for the current interaction.
  - Actions \(a \in \mathcal{A}\) are associated with feature vectors \(\mathbf{x}_{t,a} \in \mathbb{R}^d\).

- \textbf{Reward Generation}:
  - The true reward \(r_t\) for an action is modeled as:
    \[
    r_t = \mathbf{x}_{t,a}^\top \theta^* + \epsilon_t
    \]
    where \(\theta^* \in \mathbb{R}^d\) is a latent parameter vector, and \(\epsilon_t\) is Gaussian noise \(\mathcal{N}(0, \sigma^2)\) to simulate real-world uncertainty.
  - Rewards are normalized to lie within the range \([0, 1]\).

- \textbf{Non-Linear Interactions}:
  - We introduce non-linear dependencies by applying \(\tanh\) transformations to user-item interactions, capturing more complex patterns.

- \textbf{Sparse Rewards}:
  - To simulate practical sparsity in rewards, only a subset of user-item interactions provides meaningful rewards, controlled by a sparsity mask.

\subsection{Baselines}

We compare our \textbf{HybridLinearBandit} approach against the following baselines:

\textbf{Epsilon-Greedy}:
  Selects actions randomly with probability \(\epsilon = 0.1\) and otherwise exploits the best-known action.

\textbf{Upper Confidence Bound (UCB)}:
  Balances exploration and exploitation by selecting actions with the highest upper confidence bound.

\textbf{Action Recommendation (AR)}:
  Always requests human feedback to directly guide the action selection.

\textbf{Reward Manipulation (RM)}:
  Always requests human feedback to refine the observed reward signal.

\textbf{Hybrid Feedback (HF)}:
  Dynamically switches between AR and RM based on the model’s uncertainty, leveraging entropy.

\subsection{Experiment Settings}

\textbf{Rounds and Runs}:
  Each experiment runs for \(T = 1000\) rounds, with \(5\) independent trials to account for variability.

\textbf{Hyperparameters}:
  Initial entropy threshold \(\tau_{\text{init}} = 0.5\).
  Maximum entropy threshold \(\tau_{\text{max}} = 1.5\).
  Learning rate \(\alpha = 0.1\).
  Regularization parameter \(\lambda = 0.01\).

\textbf{Evaluation Metrics}: Cumulative Reward: Measures the total reward achieved over \(T\) rounds. Cumulative Regret: The gap between the optimal reward and the agent’s reward:
    \[
    \text{Regret}_T = \sum_{t=1}^T \left( r_t^* - r_t \right)
    \]
Feedback Cost: Tracks the frequency and type of human feedback requested.

\subsection{Results and Analysis}

We report the mean cumulative rewards and regrets over \(5\) runs, along with standard deviations. Error bars are provided to show variability.

\textbf{Cumulative Rewards}:
  \textbf{HF} consistently outperforms AR and RM alone, as well as Epsilon-Greedy and UCB.
  The dynamic balance of AR for high-uncertainty exploration and RM for low-uncertainty exploitation ensures robust performance.

\textbf{Cumulative Regret}:
  \textbf{HF} achieves the lowest cumulative regret, demonstrating its efficiency in minimizing suboptimal actions over time.

\textbf{Feedback Cost}:
 Compared to AR and RM, \textbf{HF} significantly reduces feedback frequency as the model learns, reducing cognitive load while maintaining performance.

The results confirm that \textbf{HF} offers an effective and scalable approach to integrating human expertise in contextual bandits. It balances exploration and exploitation more efficiently than static feedback methods.

==> sections/potential_improvement.tex <==

\section{Method Improvement: Hybrid Feedback Mechanism}

We consider a contextual bandit setting where an agent interacts with an environment over a series of rounds \(t = 1, 2, \dots, T\). At each round \(t\):
1. A user \(u_t \in \mathcal{U}\) and a set of items \(\mathcal{A}_t = \{a_1, a_2, \dots, a_k\}\) are presented.
2. The agent selects an action \(a_t \in \mathcal{A}_t\) based on the contextual features of the user \(\mathbf{x}_{u_t}\) and items \(\mathbf{x}_{a_t}\).
3. A reward \(r_t\) is observed, reflecting the user’s interaction with the selected item. The goal is to maximize the cumulative reward \(\sum_{t=1}^T r_t\).

In this framework, human feedback can be leveraged to enhance learning efficiency by providing additional information about the user's preferences.
\subsection{Hybrid Feedback Mechanism}

We introduce a \textbf{Hybrid Feedback Mechanism} that dynamically combines two types of human feedback:

- \textbf{Action Recommendation (AR)}: The human expert suggests the most suitable action when the model's uncertainty is high.

- \textbf{Reward Manipulation (RM)}: The human expert modifies the reward signal to correct the agent's evaluation of the selected action in low-uncertainty settings.

\subsection{Entropy-Based Decision for Feedback}

To determine when to request feedback and which type to use, we utilize the \textbf{entropy} of the predicted action probabilities:
\[
H(\mathbf{p}) = - \sum_{i=1}^{k} p(a_i) \log p(a_i)
\]
Where \(p(a_i)\) is the probability of selecting action \(a_i\).

\textbf{High Entropy} (\(H(\mathbf{p}) > \tau_t\)): The model is uncertain, and AR is used.

\textbf{Low Entropy} (\(H(\mathbf{p}) \leq \tau_t\)): The model is confident, and RM is applied to fine-tune reward estimates.

The threshold \(\tau_t\) evolves dynamically during training:
\[
\tau_t = \tau_{\text{init}} + \frac{t}{T} (\tau_{\text{max}} - \tau_{\text{init}})
\]
where \(\tau_{\text{init}}\) is the initial threshold, and \(\tau_{\text{max}}\) is the maximum threshold.

We propose \textbf{HybridLinearBandit}, which integrates AR and RM dynamically. The model consists of:

\textbf{Linear Model}: Parameterized by \(\theta\), updated using gradient-based learning.

\textbf{Entropy Threshold Adjustment}: Adaptively controls feedback type and frequency.



\[
\begin{array}{ll}
\hline
\multicolumn{2}{l}{\textbf{Algorithm 2: HybridLinearBandit with Dynamic Feedback}} \\
\hline
\textbf{Input:} & \text{Context } \mathbf{x}_t \in \mathbb{R}^d \text{ at round } t, \text{ action space } \mathcal{A}, \text{ total rounds } T, \\
& \text{initial entropy threshold } \tau_{\text{init}}, \text{ maximum threshold } \tau_{\text{max}}, \\
& \text{learning rate } \alpha, \text{ regularization parameter } \lambda. \\
\hline
\textbf{Initialize:} & \theta = \mathbf{0} \text{ (parameter vector)}, \tau_1 = \tau_{\text{init}} \\
\textbf{For each round } t = 1, \dots, T: & \\
& \textbf{Action Selection:} \\
& \quad \mathbf{s}_t = \{\mathbf{x}_{t,a}^\top \theta \,|\, a \in \mathcal{A}\} \quad (\text{compute scores for each action}) \\
& \quad \mathbf{p}_t = \text{Softmax}(\mathbf{s}_t) \quad (\text{compute action probabilities}) \\
& \quad a_t = \arg\max \mathbf{p}_t \quad (\text{select action with max probability}) \\
\\
& \textbf{Compute Entropy:} \\
& \quad H(\mathbf{p}_t) = -\sum_{a \in \mathcal{A}} p_t(a) \log p_t(a) \quad (\text{calculate entropy of action probabilities}) \\
\\
& \textbf{Request Feedback:} \\
& \quad \textbf{If } H(\mathbf{p}_t) > \tau_t: \\
& \quad \quad \text{Request Action Recommendation (AR)} \\
& \quad \textbf{Else:} \\
& \quad \quad \text{Request Reward Manipulation (RM)} \\
\\
& \textbf{Observe Feedback:} \\
& \quad \text{Receive feedback } r_t \text{ based on selected feedback type} \\
\\
& \textbf{Update Model:} \\
& \quad \theta \leftarrow \theta + \alpha \cdot (r_t - \mathbf{x}_{t,a_t}^\top \theta) \cdot \mathbf{x}_{t,a_t} - \lambda \theta \quad (\text{gradient update with regularization}) \\
\\
& \textbf{Adjust Entropy Threshold:} \\
& \quad \tau_t \leftarrow \tau_{\text{init}} + \frac{t}{T} (\tau_{\text{max}} - \tau_{\text{init}}) \quad (\text{dynamic adjustment}) \\
\\
\textbf{Output:} & \text{Trained parameter vector } \theta. \\
\hline
\end{array}
\]

Here is a detailed explanation for the algorithm:

1. \textbf{Action Selection}:
   - The agent uses the current model \(\theta\) to compute a score \(\mathbf{s}_t\) for each action \(a \in \mathcal{A}\) based on the context \(\mathbf{x}_t\).
   - Action probabilities \(\mathbf{p}_t\) are derived using the softmax function, balancing exploration and exploitation.

2. \textbf{Entropy Calculation}:
   - Entropy \(H(\mathbf{p}_t)\) quantifies the uncertainty in the action probabilities.

3. \textbf{Dynamic Feedback}:
   - When uncertainty (entropy) is high, request \textbf{AR} to refine action selection.
   - When uncertainty is low, use \textbf{RM} to fine-tune the reward model.

4. \textbf{Model Update}:
   - Perform gradient-based updates with regularization to minimize the loss based on the received feedback.

5. \textbf{Threshold Adjustment}:
   - The entropy threshold \(\tau_t\) dynamically increases as the agent becomes more confident, reducing feedback frequency over time.
   
\subsection{Dynamic Feedback Frequency}

The proposed mechanism dynamically adjusts feedback frequency: (i) \textbf{Early Rounds}: Frequent feedback (\(H(\mathbf{p}) > \tau_t\)) to explore the action space. (ii) \textbf{Later Rounds}: Reduced feedback as the model gains confidence, focusing on exploitation and fine-tuning.

This hybrid approach ensures efficient use of human feedback while minimizing cognitive load.


==> sections/regret_bound.tex <==
\subsection{Regret bound for contexual bandits with entropy-based human feedback}

We determine a regret bound for our proposed algorithm, focusing on entropy-based human feedback in a contextual bandit setting. The goal is to show how incorporating selective oracle feedback affects cumulative regret.


Let \(T\) be the total number of rounds, and \(\mathcal{A}\) the set of available actions. At each round \(t\): The agent observes a context \(s_t\). The agent selects an action \(a_t \in \mathcal{A}\) based on its policy \(\pi_t\), which incorporates feedback if requested. The oracle feedback is solicited when the entropy of the policy \(H(\pi_t)\) exceeds a threshold \(\lambda\). The observed reward \(r_t(a_t)\) is a combination of environment and feedback rewards.

The expected regret at time \(t\) is defined as:
\[
\text{Regret}_t = \mathbb{E}[r_t(a^*_t) - r_t(a_t)],
\]
% where \(a^*_t = \arg\max_{a \in \mathcal{A}} \mathbb{E}[r_t(a)]\) is the optimal action.
where \(a^*_t = \pi^*(s_t)\) is the optimal action.

The total regret over \(T\) rounds is:
\[
\text{Regret}(T) = \sum_{t=1}^T \text{Regret}_t.
\]


\textbf{Assume}:
The entropy threshold \(\lambda\) ensures that feedback is solicited with probability \(P(H(\pi_t) > \lambda) = p\).
Oracle feedback provides correct information with probability \(q_t\).

Then, the expected regret of the proposed algorithm is bounded by:
\[
\mathbb{E}[\text{Regret}(T)] \leq O\left(\sqrt{T |\mathcal{A}| \log T}\right) + O\left(\frac{(1 - p) T}{q_t}\right).
\]

1. Regret Decomposition:
   Decompose regret into two components:
   \[
   \text{Regret}(T) = \sum_{t \in \mathcal{F}} \text{Regret}_t + \sum_{t \notin \mathcal{F}} \text{Regret}_t,
   \]
   where \(\mathcal{F}\) is the set of rounds where feedback is requested (\(H(\pi_t) > \lambda\)).

2. Regret Without Feedback (\(t \notin \mathcal{F}\)):
   When no feedback is requested, the regret follows standard contextual bandit regret:
   \[
   \mathbb{E}[\text{Regret}_{\text{no-feedback}}(T)] \leq O(\sqrt{T |\mathcal{A}| \log T}).
   \]

3. Regret With Feedback (\(t \in \mathcal{F}\)):
   For rounds where feedback is solicited: (i) Feedback improves decision quality, reducing regret proportional to feedback accuracy \(q_t\). (ii) The regret in feedback rounds is bounded by \((1 - q_t)\) per round:
   \[
   \mathbb{E}[\text{Regret}_{\text{feedback}}(T)] \leq O\left(\frac{(1 - p) T}{q_t}\right).
   \]

4. Combining Terms:
   Combining both terms yields the total regret bound:
   \[
   \mathbb{E}[\text{Regret}(T)] \leq O\left(\sqrt{T |\mathcal{A}| \log T}\right) + O\left(\frac{(1 - p) T}{q_t}\right).
   \]


We have the following implications:

- Feedback Benefit: The bound highlights how oracle feedback reduces regret by improving decision-making in high-uncertainty rounds.

- Trade-off: The second term reflects the cost-benefit trade-off of feedback. With frequent and accurate feedback (\(p \to 1\) and \(q_t \to 1\)), the regret decreases significantly.

- Entropy Threshold: The choice of \(\lambda\) (affecting \(p\)) allows control over feedback frequency, balancing feedback cost and regret reduction.

==> sections/theoretical_proof.tex <==





\section{Trade-offs Between Action Recommendation and Reward Manipulation Using Lower Bounds}
We can incorporate a lower bound analysis to compare the trade-offs between Action Recommendation (AR) and Reward Manipulation (RM). It highlights the theoretical benefits and limitations of each feedback type.


\textbf{Problem Setup and Notation}

Let:
\( T \): Total number of rounds.
\( K \): Number of actions.
\( \mathcal{A} \): Action space.
\( s_t \): Context observed at round \( t \).
\( r_t(a) \): Reward for action \( a \) at round \( t \).
\( q_t^{AR} \): Probability that the feedback in AR is correct (expert recommendation quality).
\( q_t^{RM} \): Probability that the reward signal is correctly modified in RM (expert reward quality).
\( p_t \): Probability of querying feedback in either AR or RM.

We aim to derive regret lower bounds for both feedback types and analyze their trade-offs.


\subsection{Action Recommendation (AR)}

In the AR setting: The agent queries the oracle to receive the recommended action \( a_t^{AR} \), which is assumed to be correct with probability \( q_t^{AR} \).

\textbf{Regret Lower Bound for AR}

In rounds where feedback is not queried (\( 1 - p_t \)), the regret follows standard contextual bandit bounds:
\[
\mathbb{E}[\text{Regret}_{\text{no-feedback}}(T)] \geq O((1 - p_t) \sqrt{T K}).
\]

In rounds where AR feedback is queried (\( p_t \)), regret depends on the quality of the recommended action:
\[
\mathbb{E}[\text{Regret}_{\text{feedback}}^{AR}(T)] \geq O\left(\frac{p_t T}{q_t^{AR}}\right).
\]

Thus, the total regret for AR is bounded by:
\[
\mathbb{E}[\text{Regret}^{AR}(T)] \geq O((1 - p_t) \sqrt{T K}) + O\left(\frac{p_t T}{q_t^{AR}}\right).
\]

\subsection{Reward Manipulation (RM)}

In the RM setting: The agent receives a modified reward signal \( \tilde{r}_t(a_t) \), adjusted by the oracle to reflect feedback quality \( q_t^{RM} \).

\textbf{Regret Lower Bound for RM}

Without feedback (\( 1 - p_t \)):
\[
\mathbb{E}[\text{Regret}_{\text{no-feedback}}(T)] \geq O((1 - p_t) \sqrt{T K}).
\]

With RM feedback (\( p_t \)), the manipulated reward provides improved reward estimates, reducing regret:
\[
\mathbb{E}[\text{Regret}_{\text{feedback}}^{RM}(T)] \geq O\left(\frac{p_t T}{q_t^{RM}}\right).
\]

Thus, the total regret for RM is:
\[
\mathbb{E}[\text{Regret}^{RM}(T)] \geq O((1 - p_t) \sqrt{T K}) + O\left(\frac{p_t T}{q_t^{RM}}\right).
\]


\subsection{Trade-off Analysis}

\textbf{1. Feedback Quality \(q_t^{AR}\) vs. \(q_t^{RM}\)}:
   \textbf{AR} directly impacts action selection, which may lead to larger regret reduction if \(q_t^{AR}\) is high.
   \textbf{RM} improves the reward signal, which may be less direct but still effective in guiding future decisions.

\textbf{2. Feedback Frequency \(p_t\)}:
   Both AR and RM benefit from higher feedback frequency \(p_t\). However, querying feedback comes with costs, and the choice depends on the relative quality of feedback \(q_t\).

\textbf{3. Cumulative Regret}:
   If \(q_t^{AR} > q_t^{RM}\), AR is more effective in reducing regret:
     \[
     \mathbb{E}[\text{Regret}^{AR}(T)] < \mathbb{E}[\text{Regret}^{RM}(T)].
     \]
   Conversely, if \(q_t^{RM}\) is higher, RM could achieve lower regret.

\subsection{Practical Implications}
\textbf{When to Use AR}:
 (i) When action recommendations are highly reliable (\(q_t^{AR} \to 1\)).
 (ii) When immediate corrective feedback on actions is critical.

\textbf{When to Use RM}:
 (i) When action recommendations are less reliable, but reward signals can be improved consistently (\(q_t^{RM} > q_t^{AR}\)).
 (ii) When reward shaping can better guide learning in uncertain environments.


This analysis shows that the choice between AR and RM depends on the quality and frequency of feedback. Both methods have distinct strengths, and their trade-offs can be quantified using the derived regret bounds. Future work could further explore hybrid strategies that dynamically balance AR and RM based on real-time feedback quality.


==> sections/todolist.tex <==
% \section{TODO List for the paper}
% \begin{itemize}[label=$\square$]
%     % \item[$\checkmark$] Implement neural bandit strategies 
%     % \item[$\checkmark$]  How the work articulates with current RLHF literature and whether RLHF algorithms with discount factor $0$ are applicable?
%     % \item[$\checkmark$]   Decide whether to keep linear UCB as a comparison algorithm since, we need to compare it with other algorithms with linearzied strategies. (not important since we are using non-linear version of other algorithms, so better to remove it)
%     % \item[$\checkmark$] Rewrite the methodology section with more detail and scientific notations. 
%     % \item[$\checkmark$]  Implement TAMER framework, which will act as a baseline for CBHF by setting the discount factor to $0$
%     \item use references to ground the proposed variation and highlight the novelty of the approach 
%     \item lack of relevancy of RL with bandit approach (may be focus only on the bandit approach without explicitly referencing rlhf framework)
%     % \item[$\checkmark$] The difference between implicit feedback and preference based feedback is not presented.
%     \item Justification of obtaining feedback every 200 and 600 epochs, and a pseudo code of the algorithm to justify where to incorporate the entropy based setup. \textbf{a small experimens on 200, 300, and etc. (In the main paper, one line. Add experiments to appendix)}
%     \item \textbf{IMPORTANT} Why does the community need specific literature on bandits with human feedback, what’s the added value compared to RLHF strategies, and why isn’t it enough to set the discount factor of RLHF to 0? \textbf{We can set the discount factor RLHF to 0.} Has the idea of using entropy been explored in RLHF, and bandits with HF? \textbf{Idea of using entropy is new. Reviewers' main concern: why do we care about entropy based method?}
%     \item The quality of human feedback is not correlated with the learner’s final performance provide more intuition on why this is observed empirically
%     \item elaborate on why entropy based methods achieve good empirical performance. 
%     % \item[$\checkmark$] Why do you use a random forest classifier to generate different levels of expert quality? Can you not simply generate synthetic experiments where the level of quality is chosen uniformly at random?
%     \item \textcolor{red}{Make the method Incorporating human Feedback part more scientific, More elaborations on entropy based action restriction}
%     \item Fix the tables and figures, missing references.
%     % \item[$\checkmark$] Third item (checked)
% \end{itemize}

